Quantum rates in dissipative systems with spatially varying friction

We investigate whether making the friction spatially dependent on the reaction coordinate introduces quantum effects into the thermal reaction rates for dissipative reactions. Quantum rates are calculated using the numerically exact multi-configuration time-dependent Hartree (MCTDH) method, as well as the approximate ring-polymer molecular dynamics (RPMD), ring-polymer instanton (RPI) methods, and classical mechanics. By conducting simulations across a wide range of temperatures and friction strengths, we can identify the various regimes that govern the reactive dynamics. At high temperatures, in addition to the spatial-diffusion and energy-diffusion regimes predicted by Kramer's rate theory, a (coherent) tunnelling-dominated regime is identified at low friction. At low temperatures, incoherent tunnelling dominates most of Kramer's curve, except at very low friction when coherent tunnelling becomes dominant. Unlike in classical mechanics, the bath's influence changes the equilibrium time-independent properties of the system, leading to a complex interplay between spatially dependent friction and nuclear quantum effects even at high temperatures. More specifically, a realistic friction profile can lead to an increase (decrease) of the quantum (classical) rates with friction within the spatial-diffusion regime, showing that classical and quantum rates display qualitatively different behaviours. Except at very low frictions, we find that RPMD captures most of the quantum effects in the thermal reaction rates.

==> abstract.tex <==


We investigate whether making the friction spatially dependent \rev{on the reaction coordinate} introduces quantum effects into the thermal reaction rates for dissipative reactions. \rev{Quantum rates are calculated}  using the numerically exact multi-configuration time-dependent Hartree (MCTDH) method, as well as the approximate ring-polymer molecular dynamics (RPMD), ring-polymer instanton (RPI) methods, and classical molecular dynamics. 
By conducting simulations across a wide range of temperatures and friction strengths, we can identify the various regimes that govern the reactive dynamics. At high temperatures, in addition to the {spatial-diffusion} and  {energy-diffusion} regimes predicted by Kramer's rate theory, a (coherent) {tunnelling-dominated} regime is identified at low friction. At low temperatures, incoherent tunnelling dominates most of Kramer's curve, except at very low friction when coherent tunnelling becomes dominant.
Unlike in classical mechanics, the bath's influence changes the equilibrium time-independent properties of the system, leading
to a complex interplay between spatially dependent friction and nuclear quantum effects even at high temperatures. %Classical and quantum rates display qualitatively different behaviours in some scenarios, even at high temperatures. 
More specifically, a realistic friction profile can lead to an increase (decrease) of the quantum (classical) rates with friction within the {spatial-diffusion} regime, showing that classical and quantum rates display qualitatively different behaviours.
%We find that the spatial dependence of the friction introduces large quantum effects across the full range of frictions studied. However, these effects are quantum dynamical only at very low frictions; at higher frictions, they arise mainly from changes to the free-energy profile brought about by coupling between quantum thermal fluctuations of the system with the bath.
Except at very low frictions, we find that RPMD captures most of the quantum effects in the thermal reaction rates.




